Data-graph repairs: the preferred approach

Repairing inconsistent knowledge bases is a task that has been assessed, with great advances over several decades, from within the knowledge representation and reasoning and the database theory communities. As information becomes more complex and interconnected, new types of repositories, representation languages and semantics are developed in order to be able to query and reason about it. Graph databases provide an effective way to represent relationships among data, and allow processing and querying these connections efficiently. In this work, we focus on the problem of computing preferred (subset and superset) repairs for graph databases with data values, using a notion of consistency based on a set of Reg-GXPath expressions as integrity constraints. Specifically, we study the problem of computing preferred repairs based on two different preference criteria, one based on weights and the other based on multisets, showing that in most cases it is possible to retain the same computational complexity as in the case where no preference criterion is available for exploitation.

==> sections/computing_multiset_preferred_repairs.tex <==




\begin{table}
\begin{tabular}{|l|p{6.2cm}|p{5.375cm}|}
\hline
 & \multicolumn{1}{c|}{Subset} & \multicolumn{1}{c|}{Superset}  \\ \hline
\Gregxpath   & \begin{tabular}[c]{@{}l@{}}\textsc{NP-complete} since the problem is intractable without preferences \end{tabular} & \begin{tabular}[c]{@{}l@{}}Undecidable for fixed set of \\ path expressions (Th.~\ref{teo:supersetIndecidible}) and \\ for an unfixed set of node \\
expressions (Th.~\ref{teo:undecidabilityNodeExpressions})\end{tabular} \\
\hline
\multicolumn{1}{|c|}{\Gposregxpath} & \begin{tabular}[c]{@{}l@{}}PTime for node constraints. (Th.~\ref{teo:uniqueSubsetRepair}) \\ NP-complete in data complexity for \\ path constraints (Th.~\ref{teo:subsetPositiveIntractable}) \end{tabular} & \begin{tabular}[c]{@{}l@{}}PTime for any fixed constraints\\ (Th.~\ref{teo:tractableSuperset}) or for an unfixed set of \\ node expressions (Th.~\ref{teo:supersetPostNodeEpxressionTractable}). \\ NP-complete otherwise (Th.~\ref{teo:supsetHardInfinite}) \end{tabular} \\ \hline
\end{tabular}
\caption{Summary of the results obtained for the subset and superset repair problems.}
\label{table:1}
\end{table}

\vspace{1cm}
Mencionar que:
\begin{itemize}
    \item (subset $\weight$/multiset) como subset en reggxpath pos es NP-c (con las expresiones fijas), y lo que se demuestra ahi es que decidir si existe un repair no vacio es Np-c, entonces decidir si existe un repair preferido va a ser NP-c. 
    
    \item (subset $\weight$/multiset) Si solo se usan expresiones de nodo positivas, entonces, como hay un único subset repair (resultado de Abriolaetal2023) y se puuede obtener en PTIME, entonces es el preferido.
    
    \item (superset) El problema de decision aca era decidir si siquiera existía un superset repair (es lo mismo que usar la preferencia que le asigna peso 0 a todos). Entonces, si era NP-completo para algun conjunto de reglas L, tambien lo es encontrar uno repair preferido.
    Por lo tanto, los únicos casos que pueden ser polinomiales, son los que ya eran polinomiales. Estos casos son fragmento positivo con R fijo, o bien expresiones de nodo positivas:

    \begin{itemize}
        \item Para $\weight$: es NP-completo aun si se consideran expresiones de nodo fijas, y antes esto era tratable (incluso si no estaban fijas).

        \item Para multiset: es PTIME si se consideran expresions positivas con R fijo (Teo 49). Si R no es fijo y $Sigma_n$ puede ser infinito es NP-Hard (Teo 48 del paper viejo)
    \end{itemize}
\end{itemize}

